An Empirical Study of Intel Xeon Phi

With at least 50 cores, Intel Xeon Phi is a true many-core architecture. Featuring fairly powerful cores, two cache levels, and very fast interconnections, the Xeon Phi can get a theoretical peak of 1000 GFLOPs and over 240 GB/s. These numbers, as well as its flexibility - it can be used both as a coprocessor or as a stand-alone processor - are very tempting for parallel applications looking for new performance records. In this paper, we present an empirical study of Xeon Phi, stressing its performance limits and relevant performance factors, ultimately aiming to present a simplified view of the machine for regular programmers in search for performance. To do so, we have micro-benchmarked the main hardware components of the processor - the cores, the memory hierarchies, the ring interconnect, and the PCIe connection. We show that, in ideal microbenchmarking conditions, the performance that can be achieved is very close to the theoretical peak, as given in the official programmer's guide. We have also identified and quantified several causes for significant performance penalties. Our findings have been captured in four optimization guidelines, and used to build a simplified programmer's view of Xeon Phi, eventually enable the design and prototyping of applications on a functionality-based model of the architecture.

==> bm_methodology.tex <==
\section{Measurement Methodology} \label{sec:methodology}
In this section we present a high-level overview of the methodology used for our empirical evaluation. We include a discussion on the capabilities to be measured, the metrics that we propose, and the design of the benchmarks that allow us to isolate and measure the targeted capabilities.

\subsection{Metrics}
We use different performance metrics to evaluate Intel Xeon Phi and its components. On the whole, we divide the performance metrics into two categories: (1) latency-oriented metrics (e.g., cycles or execution time), and (2) throughput-oriented metrics (e.g., GFlops, GB/s). \textit{Latency} is the time required to perform an action or produce a result. Thus, a latency measurement focuses on a single action from the beginning to the end. Meanwhile, \textit{throughput} is the number of such actions executed or results produced per unit of time. When measuring throughput, we need to put plenty of (multi-threaded) workloads to fully occupy the target system. In contrast, the latency measurement poses higher requirements in terms of timing precision and we need to take the timing overhead into account. However, when one action depends its previous one (so that the current action has to wait until the results are available), it is straightforward to measuring latency by running a lot of such actions (e.g., measuring memory access latency by pointer-chasing). 

Considering their differences, we use two separate measurement and timing methods for latency and throughput in Listing~\ref{lst:lat_mea} and~\ref{lst:thr_mea}. Apart from the timing methods, another difference lies in the number of threads. When measuring latency, we often use a single thread (or at most two threads, for example, when measuring the latency of cacheline transfers). On the other hand, measuring throughput needs to use plenty of threads to fully utilize the cores or generate enough memory requests. In this paper, we use OpenMP to generate multiple threads. Furthermore, the latency measurement uses an \textit{instruction sequence}, which is a sequence of native instructions compiled with \texttt{-O0} option. In this way, we can avoid the interference of aid instructions (e.g., address calculation instructions) generated from a high-level code segment. The throughput measurement uses a high-level \textit{code sequence}, which is expressed in a high-level language like \textit{C}. The code sequence is compiled with \texttt{-O3} option and we need to use some techniques to avoid aggressive compiler optimizations. 

%we aim to accurately measure the execution time of a single instruction or a cache-line action.

To eliminate the effects of TLB misses and cold code caches, we repeat each run three passes and time the third pass. However, we flush the data caches between contiguous passes when they interference each other through caching data. Furthermore, we run each experiments 10 (or 1000) times, from which we obtain the \textit{median} value.


\lstdefinestyle{customc}{
  belowcaptionskip=1\baselineskip,
  breaklines=true,
  frame=L,
  xleftmargin=\parindent,
  language=C,
  showstringspaces=false,
  basicstyle=\footnotesize\ttfamily,
  keywordstyle=\bfseries\color{green!40!black},
  commentstyle=\itshape\color{purple!40!black},
  identifierstyle=\color{black},
  stringstyle=\color{orange},
  morekeywords={\#, pragma, omp, parallel},
}

\lstdefinestyle{customasm}{
  belowcaptionskip=1\baselineskip,
  frame=L,
  xleftmargin=\parindent,
  language=[x86masm]Assembler,
  basicstyle=\footnotesize\ttfamily,
  commentstyle=\itshape\color{purple!40!black},
}

\lstset{escapechar=@,style=customc}


\begin{figure*}[!t]
\centering
\resizebox{0.82\textwidth}{!}{
\begin{minipage}{0.38\textwidth}
\lstinputlisting[caption=Latency measurement,label=lst:lat_mea]{code/tm_lat.c}
\end{minipage}
\begin{minipage}{0.02\textwidth}
\end{minipage}
\begin{minipage}{0.42\textwidth}
\lstinputlisting[caption=Throughput measurement,label=lst:thr_mea]{code/tm_thr.c}
\end{minipage}}
\end{figure*}


\subsection{Micro-Benchmarks} \label{subsec:micro_ben}
When evaluating Xeon Phi, we focus on five components: (1) the vector processing cores, (2) the on-chip memory, (3) the off-chip memory, (4) the ring interconnect, and (5) the PCIe connection. Since Intel Xeon Phi inherits a lot from traditional CPUs, we reuse the existing microbenchmarks, rather than inventing new wheels. At the same time, Xeon Phi has made many architectural innovations, among which are the new vector instructions, the ring-connected last-level cache, etc. As a result, we also need to adapt the microbenchmarks to this new processor. 

\textbf{Instruction Latency and Throughput:} Agner Frog~\cite{citeulike:12589493} and Torbjorn Granlund~\cite{citeulike:12589489} measure instruction latency by running a sequence of dependent instructions. In this work, we focus on the vector processing units of Xeon Phi and thus the latency of typical vector instructions. Specifically, we roughly divide the vector instructions into five groups: mask instructions, arithmetic (logical) instructions, convert instructions, permute instructions, and maths instructions. The selected results are shown in Table~\ref{tbl:ins_lat}. Furthermore, they use similar approach to measure throughput in terms of \textit{instruction per cycle (IPC)}. However, we argue that a fully loaded measurement, that uses all the processing cores, will demonstrate more realistic significance for programmers. Thus, we use the \texttt{flops} microbenchmark in \texttt{shoc-mic}~\footnote{\url{https://github.com/vetter/shoc-mic.}} to explore the factors of reaching the theoretical flops on Xeon Phi (Section~\ref{subsec:vec_thr}). Finally, Xeon Phi supports EMU (extended maths unit) that aims only at single-precision operations. We design mirobenchmarks to show the performance differences between single-precision and double-precision operations. 



\textbf{Memory Latency:} \texttt{BenchIT}~\cite{website:benchit_benchmark} and \texttt{lmbench}~\cite{citeulike:12586247} use \textit{pointer-chasing} to measure the on-chip and off-chip memory access latency. This approach facilitates us to recognize the hierarchies of memory systems and its corresponding access latencies. Thus, we use similar approach to measure latency on Xeon Phi (Section~\ref{subsec:cache_property}). When more than two cores take part in communication, latency measurement becomes complicated. For this, Daniel Molka et al. propose an approach to quantify the cache-coherent effects~\cite{citeulike:8778343}. In our work, we adapt this approach to Xeon Phi by making two changes: (1) replace the \texttt{mfence} instruction with equivalent instructions, and (2) replace the \texttt{clflush} instruction with equivalent instructions.

\textbf{Memory Bandwidth:}  McCalphin's stream benchmarks~\cite{website:stream_benchmark} has memory bandwidth measurements and results for a large number of high-end systems. We did not use them because the measurements are based a combination of both read and write. In this paper, we want to separate \textit{read} and \textit{write} operations, and to make a bandwidth estimation for any given real scenarios. In BenchIT, Daniel Molka et al. also measure bandwidth in a similar way with that of latency measurement. But the microbenchmark needs to be compiled with the \texttt{-O0} option, and disable the software prefetching on Xeon Phi. Thus, this measurement will underestimate bandwidth. \texttt{lmbench} attempts to measure system's ability of transfer data between processor, cache, memory, disk, and network. However, lmbench supports parallelism in term of \texttt{Unix Process}, which has to use special inter-process communication methods instead of data sharing within a single data space. Thus, we present an \texttt{OpenMP} implementation to measure memory bandwidth based on the microbenchmarks in lmbench. 


\textbf{Ring Interconnect/Contention:} On Xeon Phi, all the components are connected by the ring interconnect. When multiple threads are requesting data simultaneously, the shared components like the ring stop or DTDs will possibly become performance bottlenecks. Thus, we use \textit{thread affinity} and the bandwidth microbenchmarks to quantify the bandwidth changes (in GB/s) for different scenarios. 

\textbf{PCIe Data Transfer: } PCI Express connects Xeon Phi to a host (e.g., a traditional CPU). When Xeon Phi is used as a coprocessor, all tasks and related data have be transfered back and forward between the host and the coprocessor. Regarding the frequent data transfers, it might be a performance bottleneck. Thus, we design a benchmark~\footnote{Our benchmark is based on Intel's sample code: \url{http://software.intel.com/en-us/articles/how-to-achieve-peak-transfer-rate}} to measure the data transfer bandwidth. 





